TIMER: Temporal Instruction Modeling and Evaluation for Longitudinal Clinical Records

Large language models (LLMs) have emerged as promising tools for assisting in medical tasks, yet processing Electronic Health Records (EHRs) presents unique challenges due to their longitudinal nature. While LLMs' capabilities to perform medical tasks continue to improve, their ability to reason over temporal dependencies across multiple patient visits and time frames remains unexplored. We introduce TIMER (Temporal Instruction Modeling and Evaluation for Longitudinal Clinical Records), a framework that incorporate instruction-response pairs grounding to different parts of a patient's record as a critical dimension in both instruction evaluation and tuning for longitudinal clinical records. We develop TIMER-Bench, the first time-aware benchmark that evaluates temporal reasoning capabilities over longitudinal EHRs, as well as TIMER-Instruct, an instruction-tuning methodology for LLMs to learn reasoning over time. We demonstrate that models fine-tuned with TIMER-Instruct improve performance by 7.3% on human-generated benchmarks and 9.2% on TIMER-Bench, indicating that temporal instruction-tuning improves model performance for reasoning over EHR.

==> tables/backup_long_cases.tex <==
% \onecolumn
% \begin{longtable}{|p{3.5cm}|p{5.5cm}|p{5.5cm}|}
% \hline
% \textbf{Instruction} & 
% \textbf{LongEHR-Instruct + Llama-3.1-8B-Instruct} & 
% \textbf{Llama-3.1-8B-Instruct} \\ 
% \hline
% \multirow{6}{*}{\parbox{3.5cm}{Has the patient's mixed conductive and sensorineural hearing loss in the right ear shown any improvement over time?}} & 
% \parbox{5.5cm}{
% Response: "The patient's mixed conductive and sensorineural hearing loss in the right ear was first documented on 06/14/2017. On 08/22/2018, the patient's hearing loss was described as stable asymmetric normal to moderate mixed hearing loss. On 08/03/2020, the patient's hearing loss was described as normal through 3000 Hz sloping to moderate mixed hearing loss. While the exact progression of the patient's hearing loss is not clear, it appears that the patient's hearing loss in the right ear has remained stable over the past three years. \textcolor{red}{There is no indication of improvement.}"
% } & 
% \parbox{5.5cm}{
% Response: "\textcolor{red}{The patient's mixed conductive and sensorineural hearing loss in the right ear has shown some improvement over time.} In the 06/14/2017 visit, the patient's pure tone measures showed ``Normal sloping to moderate mixed hearing loss at the right ear.'' In the 08/22/2018 visit, the patient's pure tone measures showed ``Normal through 3000 Hz sloping to moderate mixed hearing loss at the right ear.'' In the 08/03/2020 visit, the patient's pure tone measures showed ``Normal through 3000 Hz sloping to moderate mixed hearing loss at the right ear.'' The patient's hearing loss in the right ear has remained stable, but not improved, over the three visits. However, the patient's speech recognition threshold (SRT) has improved from 25 dB HL at the right ear in the 06/14/2017 visit to 25 dB HL at the right ear in the 08/22/2018 visit and 15 dB HL at the right ear in the 08/03/2020 visit, which indicates some improvement in the patient's ability to understand speech in the right ear."
% } \\ 
% \cline{2-3}
% & 
% \parbox{5.5cm}{
% Feedback: The model accurately states that the patient's mixed conductive and sensorineural hearing loss in the right ear was first documented on 06/14/2017 and describes the hearing loss as stable from 08/22/2018 to 08/03/2020. The model correctly identifies that the audiogram on 08/03/2020 indicates moderate mixed hearing loss, consistent with the previous assessment.
% } & 
% \parbox{5.5cm}{
% Feedback: \textcolor{red}{The model incorrectly states that the patient's mixed conductive and sensorineural hearing loss in the right ear has shown improvement over time.} The reference answer correctly indicates that the hearing loss has remained stable from 08/22/2018 to 08/03/2020. The model also misrepresents the SRT values, stating they improved from 25 dB HL to 15 dB HL, which is misleading as it does not accurately reflect the overall stability of the hearing loss.
% } \\ 
% \hline
% \multirow{6}{*}{\parbox{3.5cm}{The patient is concerned about his current narcotic use. What is his current regimen, and has he expressed concerns about this previously?}} & 
% \parbox{5.5cm}{
% Response: "The patient is currently taking \textcolor{red}{methadone 60 mg per day, narco 2 to 3 mg q.h.s., and Motrin 800 mg}. He has been on a narcotic for some time. In the past, he had tried fentanyl patches, Vicodin, and morphine. He has expressed a concern about being on narcotics for the rest of his life, and would like to be weaned off of his methadone. He has also stated that he has had to increase his medication for a few days after moving, as he was unable to stand on his left leg much. He has been to another pain doctor in the past five years, Dr. Trout, and has also seen Dr. Galli. He is currently seeing Dr. Amling at the Stanford Pain Management Center. He is motivated to be weaned off of his methadone and tried on new medications."
% } & 
% \parbox{5.5cm}{
% Response: "The patient is currently taking \textcolor{red}{methadone 60 mg per day, and narco 2 to 3 mg q.h.s}. He has expressed a concern about his narcotic use, stating that he has a fear of being on narcotics for the rest of his life and would like to be weaned off of his methadone. He has previously tried to take his medication differently than prescribed by his doctors while he was moving, because he was not able to stand up on his left leg much. He has also stated that he has tried to wean off of his methadone in the past, but was unable to do so. He has also stated that he has tried to wean off of his methadone in the past, but was unable to do so. He has also stated that he has tried to wean off of his methadone in the past, but was unable to do so. He has also stated that he has tried to wean off of his methadone in the past, but was unable to do so. He has also stated that he has tried to wean off of his methadone in the past, but was unable to do so. He has also stated that he has""
% } \\ 
% \cline{2-3}
% & 
% \parbox{5.5cm}{
% Feedback: \textcolor{red}{The model accurately states the patient's current medication regimen, including Methadone 60 mg daily, Narco 2-3 mg at bedtime, and Motrin 800 mg}. It correctly notes the patient's concerns about long-term narcotic use and his desire to be weaned off Methadone, aligning with the reference answer.,
% } & 
% \parbox{5.5cm}{
% Feedback:\textcolor{red}{The model incorrectly states the patient's current narcotic regimen as Methadone 60 mg per day and Narco 2-3 mg q.h.s. }However, the reference answer specifies that the patient takes Methadone 60 mg daily, Narco 2-3 mg at bedtime, and Motrin 800 mg as needed. Additionally, the model response contains repetitive phrases about the patient's attempts to wean off Methadone, which detracts from clarity and accuracy..}\\ 
% \hline
% \multirow{6}{*}{\parbox{3.5cm}{The patient had a left knee injury in July 2022. Summarize the findings from his x-rays over time.}} & 
% \parbox{5.5cm}{
% Response: "1. \textcolor{red}{Initial x-rays on 07/18/2022} showed a subtle irregularity along the proximal tibial metaphysis on lateral view, raising concern for an occult proximal tibia fracture. 2. Repeat x-rays on 07/25/2022 showed no obvious bony abnormality, but there was soft tissue swelling in the area of tenderness. 3. Repeat x-rays on 08/22/2022 showed sclerosis across the proximal tibial metaphysis and a lateral periosteal reaction, consistent with a healing nondisplaced fracture in this location. The joint spaces of the knee were preserved, and the soft tissues were radiographically normal. 4. No further x-rays were mentioned in the provided EHR for the left knee after 08/22/2022. 5. The patient was advised to limit his weightbearing activity based on his symptoms, and follow-up was recommended in 2 weeks if he was not comfortably walking without a limp. 6. The patient was also advised to avoid high-risk activities such as going to the playground, bouncy houses, or trampolines. 7. Follow-up x-rays were recommended in 3 weeks if the patient had not returned to full running"
% } & 
% \parbox{5.5cm}{
% Response: "The patient had a left knee injury in July 2022. Over time, the x-rays showed the following findings: \n1. \textcolor{red}{Initially, there was a subtle irregularity along the proximal tibial metaphysis on lateral view X-ray on July 6, 2022, which raised concern for an occult proximal tibia fracture}.\n2. Repeat x-rays on July 25, 2022, did not show any obvious bony abnormality, but there was soft tissue swelling in the area of tenderness.\n3. Repeat x-rays on August 22, 2022, showed moderate sclerosis across the proximal tibial metaphysis as well as lateral periosteal reaction consistent with a healing nondisplaced fracture in this location. The joint spaces of the knee were preserved, and the soft tissues were radiographically normal. This confirmed the initial suspicion of a nondisplaced fracture of the proximal tibia. """Answered correctly""" \\
% """Answered correctly""" \\
% """Answered correctly""" \\
% """Answered correctly""" \\
% """Answered correctly""" \\
% """Answered correctly""" \\
% """Answered correctly""" \\
% """Answered correctly""" \\
% """Answered correctly""" \\
% """Answered correctly""" \\
% """Answered correctly"""" 
% } \\ 
% \cline{2-3}
% & 
% \parbox{5.5cm}{
% Feedback: The model accurately describes the findings from the x-rays over time, including the initial irregularity, the repeat x-ray findings, and the final assessment of the healing nondisplaced fracture. The temporal relationships are correctly represented, and the dates mentioned align with the EHR data.
% } & 
% \parbox{5.5cm}{
% \textcolor{red}{The model response contains factual inaccuracies regarding the timeline of x-ray findings. It incorrectly states that the initial x-ray was on July 6, 2022, while the correct date is July 18, 2022}. Additionally, it misrepresents the findings on July 25, 2022, as showing soft tissue swelling, which was not mentioned in the reference answer.}\\ 
% \hline
% \multirow{6}{*}{\parbox{3.5cm}{The patient was seen on 02/13/2017 for a left ankle sprain. Summarize the treatment plan and outcome at his follow-up appointments.}} & 
% \parbox{5.5cm}{
% Response: "\textcolor{red}{At the follow-up visit on 01/23/2017, the patient was placed in a lace-up ankle brace for the next week. After a week of full-time wear, the brace was to be taken off only to shower and sleep. The patient was to wean out of the brace at home and discontinue it if he remained pain-free. He was advised to avoid physical education for the next week and was told that if the limp persisted or he continued to favor the ankle after 3 weeks, he should return to the clinic. At the follow-up visit on 02/13/2017,} the patient's limp had improved, and he had full ankle range of motion without pain. He was no longer tender over the ATFL, CFL, or deltoid ligament. The plan was to refer him for physical therapy if the pain or limp persisted. The patient was advised to continue using the ankle brace as needed. The patient was able to return to physical education and was expected to get away from the brace. He was advised to follow up as needed."
% } & 
% \parbox{5.5cm}{
% Response: "\textcolor{red}{The patient was seen on 02/13/2017 for a left ankle sprain. At his follow-up appointment on 01/23/2017}, the patient was placed in a lace-up ankle brace for the next week. After a week of full-time wear, he was instructed to wean out of it at home, and if he remained pain-free, he could discontinue the brace. He was also advised to avoid physical education for the next week and to return to the clinic if he continued to favor the ankle after 3 weeks. At his follow-up appointment on 02/13/2017, the patient had improved significantly, with only a slight limp and no pain. The doctor decided that the patient did not require a prescription for physical therapy at that point and instructed him to continue to use the brace as needed. The patient was advised to follow up on an as-needed basis. The patient was seen on 02/14/2017 for a follow-up visit, but the note does not mention any new treatment plan or outcome. The patient was seen on 09/28/2017 for a gastroenterology visit, which is not related to his ankle injury. The patient was seen on 10/22/201"
% } \\ 
% \cline{2-3}
% & 
% \parbox{5.5cm}{
% Feedback: The model accurately describes the treatment plan and outcomes for the patient's follow-up appointments, including the transition from a short leg walking cast to a lace-up ankle brace and the patient's improvement in symptoms.,
% } & 
% \parbox{5.5cm}{
% Feedback:The model response contains factual inaccuracies regarding the timeline and treatment details. It states that the patient was seen on 01/23/2017 for follow-up and placed in a lace-up ankle brace, but it fails to mention that the patient was initially treated with a short leg walking cast for 3 weeks starting from 12/28/2016. Additionally, the model incorrectly states that the follow-up on 02/13/2017 showed only a slight limp, while the reference answer indicates that the patient had full ankle range of motion and good strength.}\\ 
% \hline

% \end{longtable}

==> tables/backup_main.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% medalign %%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[t]
\centering
\caption{Performance comparison (\%) of medical and general domain LLMs on MedAlign Benchmark: short vs. long context analysis.}
\label{tab:medalign-performance}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lc|cc|ccccc}
\toprule
\multirow{2.5}{*}{\bf Model} & \multirow{2.5}{*}{\bf Open Source} &\multicolumn{2}{c|}{{\cellcolor{maroon}}{\bf LLM-as-a-Judge}} &  \multicolumn{5}{c}{\cellcolor{lightblue}{\bf Standard NLP Metrics}}\\
\cmidrule(lr){3-4} \cmidrule(lr){5-9} 
& & {Correctness$\uparrow$} & {Completeness$\uparrow$} & {BERTScore$\uparrow$} & {METEOR$\uparrow$} & {chrF++$\uparrow$} & {GoogleBLEU$\uparrow$} & {ROUGE-L$\uparrow$} \\
\midrule
\rowcolor{gray!15}\multicolumn{9}{l}{\emph{Standard Medical LLM (Context Length $\leq$ 8k)}}  \\
MMed-Llama-3-8b &\cmark & 0.092 & 0.043 & 0.656 & 0.102 & 13.210 & 0.018 & 0.049 \\
meditron-7b &\cmark & 0.036 & 0.013 & 0.606 & 0.062 & 11.099 & 0.012 & 0.031 \\
MedAlpaca & \cmark& 0.130 & 0.043 & 0.659 & 0.076 & 11.304 & 0.023 & 0.048 \\
PMC-Llama-13b &\cmark & 0.119 & 0.046 & 0.660 & 0.067 & 8.838 & 0.017 & 0.037  \\
AlpaCare & \cmark & 0.271 & 0.132 & 0.665 & 0.177 & 20.390 & 0.055 & 0.113  \\
MedLM-large & \xmark & 0.413 & 0.208 & 0.759 & 0.194 & 21.990 & 0.067 & 0.138 \\
\midrule
\rowcolor{gray!15}\multicolumn{9}{l}{\emph{Long-Context General LLMs (Context Length $>$ 8k})}  \\
Mistral-7B & \cmark& 0.508 & 0.310 & 0.763 & 0.224 & 24.321 & 0.075 & 0.141 \\
Llama3.1-8b-Instruct &\cmark & 0.465 & 0.297 & 0.705 & 0.179 & 19.632 & 0.033 & 0.085 \\
\midrule
\rowcolor{gray!15}\multicolumn{9}{l}{\emph{Long-Context Medical LLMs (Context Length $>$ 8k)}}  \\
MedLM-medium &\xmark & 0.505 & 0.294 & 0.756 & 0.178 & 20.510 & 0.066 & 0.132 \\
Llama3.1-8b-Instruct+MedQA &\cmark & 0.459 & 0.277 & 0.709 & 0.193 & 20.664 & 0.036 & 0.087 \\
\rowcolor{green!10} {\instruct} & \cmark& \textbf{0.535} & \textbf{0.366} & \textbf{0.767} & \textbf{0.235} & \textbf{25.430} & \textbf{0.079} & \textbf{0.146} \\
\bottomrule
\end{tabular}
}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%% temporal eval %%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[h]
\centering
\caption{Performance comparison (\%) of medical and general domain LLMs on {\benchmark} Benchmark: short vs. long context analysis.}
\label{tab:longehr-performance}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lc|cc|ccccc}
\toprule
\multirow{2.5}{*}{\bf Model} & \multirow{2.5}{*}{\bf Open Source} &\multicolumn{2}{c|}{{\cellcolor{maroon}}{\bf LLM-as-a-Judge}} &  \multicolumn{5}{c}{\cellcolor{lightblue}{\bf Standard NLP Metrics}}\\
\cmidrule(lr){3-4} \cmidrule(lr){5-9} 
& & {Correctness$\uparrow$} & {Completeness$\uparrow$} & {BERTScore$\uparrow$} & {METEOR$\uparrow$} & {chrF++$\uparrow$} & {GoogleBLEU$\uparrow$} & {ROUGE-L$\uparrow$} \\
\midrule
\rowcolor{gray!15}\multicolumn{9}{l}{\emph{Standard Medical LLM (Context Length $\leq$ 8k)}}  \\
MMed-Llama-3-8b &\cmark & 0.310 & 0.168 & 0.721 & 0.213 & 24.146 & 0.054 & 0.103 \\
meditron-7b &\cmark & 0.102 & 0.033 & 0.642 & 0.093 & 16.549 & 0.030 & 0.053 \\
MedAlpaca & \cmark & 0.178 & 0.053 & 0.556 & 0.014 & 1.382 & 0.004 & 0.003 \\
PMC-Llama-13b &\cmark & 0.040 & 0.017 & 0.257 & 0.018 & 2.499 & 0.007 & 0.012 \\
AlpaCare & \cmark & 0.059 & 0.036 & 0.180 & 0.055 & 6.048 & 0.024 & 0.036 \\
MedLM-large & \xmark & 0.446 & 0.238 & 0.838 & 0.340 & 36.477 & 0.189 & 0.280 \\
\midrule
\rowcolor{gray!15}\multicolumn{9}{l}{\emph{Long-Context General LLMs (Context Length $>$ 8k})}  \\
Mistral-7B & \cmark & 0.439 & 0.424 & 0.528 & 0.262 & 27.023 & 0.119 & 0.160 \\
Llama3.1-8b-Instruct &\cmark & 0.554 & 0.540 & 0.799 & 0.382 & 38.323 & 0.111 & 0.182 \\
\midrule
\rowcolor{gray!15}\multicolumn{9}{l}{\emph{Long-Context Medical LLMs (Context Length $>$ 8k)}}  \\
MedLM-medium &\xmark & \underline{0.700} & 0.459 & \textbf{0.853} & \underline{0.417} & \underline{43.156} & \textbf{0.234} & \textbf{0.307} \\
Llama3.1-8b-Instruct+MedQA &\cmark & 0.601 & \underline{0.597} & 0.801 & 0.385 & 39.031 & 0.119 & 0.195 \\
\rowcolor{green!10} {\instruct} & \cmark & \textbf{0.789} & \textbf{0.611} & \underline{0.845} & \textbf{0.429} & \textbf{45.110} & \underline{0.204} & \underline{0.274} \\
\bottomrule
\end{tabular}
}
\end{table*}



==> tables/new_results_main.tex <==
\begin{table*}[t]
\centering
\caption{Performance (\%) of baseline models and \instruct on MedAlign and \benchmark benchmarks, reported as mean ± standard deviation from bootstrap resampling (n=10,000) over the test set with 100 samples.}
\label{tab:instruct-performance}
\renewcommand{\arraystretch}{0.88}
\resizebox{\linewidth}{!}{
\begin{tabular}{p{5cm}|cccc|cccc}
\toprule
\multirow{4}{*}{\textbf{Model Name}} & \multicolumn{4}{c|}{\textbf{MedAlign}} & \multicolumn{4}{c}{\textbf{\benchmark}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& \multicolumn{2}{c}{\cellcolor{yellow}LLM-as-Judge} & \multicolumn{2}{c|}{\cellcolor{lightblue}Automatic Metrics} & \multicolumn{2}{c}{\cellcolor{yellow}LLM-as-Judge} & \multicolumn{2}{c}{\cellcolor{lightblue}Automatic Metrics} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
& Correct & Complete & BERTScore & ROUGE-L & Correct & Complete & BERTScore & ROUGE-L \\
\midrule
\rowcolor{gray!10}\multicolumn{9}{l}{\textbf{Existing Medical Finetuned Model}}  \\
\addlinespace[2pt]
Meditron-7B\textsuperscript{*}  & 4.76  {\scriptsize $\pm$ 2.81} & 1.73 {\scriptsize$\pm$ 1.52} & 60.47 {\scriptsize$\pm$ 1.40} & 3.27 {\scriptsize$\pm$ 0.60} & 2.99 {\scriptsize$\pm$ 1.62} & 1.00 {\scriptsize$\pm$ 0.87} & 65.23 {\scriptsize$\pm$ 1.00} & 5.39 {\scriptsize$\pm$ 0.61} \\
MedAlpaca\textsuperscript{*} & 16.88 {\scriptsize$\pm$ 4.76} & 5.63 {\scriptsize$\pm$ 2.81} & 65.98 {\scriptsize$\pm$ 1.20} & 5.14 {\scriptsize$\pm$ 1.20} & 7.21 {\scriptsize$\pm$ 2.49} & 1.49 {\scriptsize$\pm$ 1.12} & 72.06 {\scriptsize$\pm$ 0.74} & 9.25 {\scriptsize$\pm$ 0.79} \\
AlpaCare\textsuperscript{*} & 34.63 {\scriptsize$\pm$ 6.06} & 16.45 {\scriptsize$\pm$ 4.76} & 67.05 {\scriptsize$\pm$ 3.30} & 11.77 {\scriptsize$\pm$ 1.40} & 7.71 {\scriptsize$\pm$ 2.61} & 1.24 {\scriptsize$\pm$ 1.12} & 75.07 {\scriptsize$\pm$ 0.10} & 14.39 {\scriptsize$\pm$ 0.75} \\
MMed-LLaMA-3-8B\textsuperscript{*}  & 11.69 {\scriptsize$\pm$ 4.11} & 5.63 {\scriptsize$\pm$ 2.81} & 65.76 {\scriptsize$\pm$ 0.80} & 5.01 {\scriptsize$\pm$ 1.10} & 17.66 {\scriptsize$\pm$ 3.73} & 6.72 {\scriptsize$\pm$ 2.36} & 72.77 {\scriptsize$\pm$ 0.55} & 10.80 {\scriptsize$\pm$ 0.60} \\
PMC-LLaMA-13B\textsuperscript{*} & 15.15 {\scriptsize$\pm$ 4.55} & 5.63 {\scriptsize$\pm$ 2.81} & 65.04 {\scriptsize$\pm$ 1.40} & 3.79 {\scriptsize$\pm$ 0.70} & 1.24 {\scriptsize$\pm$ 1.12} & 0.50 {\scriptsize$\pm$ 0.62} & 29.17 {\scriptsize$\pm$ 2.81} & 0.77 {\scriptsize$\pm$ 0.35} \\
MedLM-Large\textsuperscript{*}\textsuperscript{†}  & 52.81 {\scriptsize$\pm$ 6.49} & 26.41 {\scriptsize$\pm$ 5.63} & 77.04 {\scriptsize$\pm$ 0.84} & 14.76 {\scriptsize$\pm$ 1.53} & 22.44 {\scriptsize$\pm$ 4.11} & 8.73 {\scriptsize$\pm$ 2.75} & 82.19 {\scriptsize$\pm$ 0.44} & 22.43 {\scriptsize$\pm$ 1.16} \\
MedLM-Medium\textsuperscript{†}  & 63.20 {\scriptsize$\pm$ 6.28} & 37.66 {\scriptsize$\pm$ 6.06} & 76.40 {\scriptsize$\pm$ 0.92} & 14.26 {\scriptsize$\pm$ 1.61} & 47.76 {\scriptsize$\pm$ 4.73} & 22.64 {\scriptsize$\pm$ 4.10} & 83.27 {\scriptsize$\pm$ 0.47} & 24.33 {\scriptsize$\pm$ 1.26} \\
MedInstruct\textsuperscript{‡}  & 59.74 {\scriptsize$\pm$ 6.28} & 35.93 {\scriptsize$\pm$ 6.06} & 71.60 {\scriptsize$\pm$ 0.81} & 9.11 {\scriptsize$\pm$ 0.77} & 59.45 {\scriptsize$\pm$ 4.73} & 38.81 {\scriptsize$\pm$ 4.73} & 80.14 {\scriptsize$\pm$ 0.47} & 18.86 {\scriptsize$\pm$ 0.73} \\
% \midrule
% \rowcolor{gray!10}\multicolumn{11}{l}{\textbf{Instruct-Tuned Models w/ Short Form vs. Longitudinal Instructions (Context Length $>$ 8k)}}  \\
\midrule
% \rowcolor{gray!10}\multicolumn{9}{l}{\textbf{General Long Context Model}}  \\
\rowcolor{gray!10}\multicolumn{9}{l}{\textbf{\textsc{\instruct} Tuned Model with Different Base}}  \\
\addlinespace[2pt]
Qwen2.5-7B-Instruct  & 71.00 {\scriptsize$\pm$ 5.84} & 52.81 {\scriptsize$\pm$ 6.49} & 73.59 {\scriptsize$\pm$ 0.60} & 9.73 {\scriptsize$\pm$ 0.70} & 67.41{\scriptsize$\pm$4.48} & 53.48{\scriptsize$\pm$4.85} & 80.81{\scriptsize$\pm$0.34} & 18.40{\scriptsize$\pm$0.64} \\
\rowcolor{green!10}w/ \textsc{\instruct} Tuning  & 73.16 {\scriptsize$\pm$ 5.63} & 53.25 {\scriptsize$\pm$ 6.49} & 72.82 {\scriptsize$\pm$ 0.60} & 8.26 {\scriptsize$\pm$ 0.60} & 69.15{\scriptsize$\pm$4.48} & 52.99{\scriptsize$\pm$4.85} & 81.53{\scriptsize$\pm$0.35} & 19.12{\scriptsize$\pm$0.66} \\
Llama3.1-8B-Instruct  & 55.41 {\scriptsize$\pm$ 6.28} & 36.80 {\scriptsize$\pm$ 6.06} & 70.48 {\scriptsize$\pm$ 0.80} & 8.73 {\scriptsize$\pm$ 0.90} & 57.96 {\scriptsize$\pm$ 4.85} & 34.58 {\scriptsize$\pm$ 0.46} & 79.49 {\scriptsize$\pm$ 0.45} & 17.78 {\scriptsize$\pm$ 0.70} \\
\rowcolor{green!10} w/ \textsc{\instruct} Tuning  & 65.80 {\scriptsize$\pm$ 6.06} & 45.89 {\scriptsize$\pm$ 6.49} & 76.50 {\scriptsize$\pm$ 0.80} & 14.60 {\scriptsize$\pm$ 1.40} & 64.68 {\scriptsize$\pm$ 4.73} & 46.27 {\scriptsize$\pm$ 4.85} & 83.20 {\scriptsize$\pm$ 0.40} & 22.60 {\scriptsize$\pm$ 1.07} \\
% \midrule
% \rowcolor{gray!10}\multicolumn{9}{l}{\textbf{\textsc{\instruct} Tuned Model}}  \\
% \addlinespace[2pt]
\bottomrule
\multicolumn{9}{l}{\small 
\textsuperscript{*}These models have a maximum context length $\leq$ 8K. We truncated the most recent records to fit within their maximum size.} \\
\multicolumn{9}{l}{\small 
\textsuperscript{†}MedLM are powered by Med-PaLM 2, which is a medical fine-tuned version of Google PaLM.} \\
\multicolumn{9}{l}{\small 
\textsuperscript{‡}We instruct-tuned MedInstruct w/ Llama3.1-8B-Instruct as the base model.}
\end{tabular}
}
\vskip -1.5em
\end{table*}

